From Explanation to Action: An End-to-End Human-in-the-loop Framework for Anomaly Reasoning and Management

Anomalies are often indicators of malfunction or inefficiency in various systems such as manufacturing, healthcare, finance, surveillance, to name a few. While the literature is abundant in effective detection algorithms due to this practical relevance, autonomous anomaly detection is rarely used in real-world scenarios. Especially in high-stakes applications, a human-in-the-loop is often involved in processes beyond detection such as verification and troubleshooting. In this work, we introduce ALARM (for Analyst-in-the-Loop Anomaly Reasoning and Management); an end-to-end framework that supports the anomaly mining cycle comprehensively, from detection to action. Besides unsupervised detection of emerging anomalies, it offers anomaly explanations and an interactive GUI for human-in-the-loop processes -- visual exploration, sense-making, and ultimately action-taking via designing new detection rules -- that help close ``the loop'' as the new rules complement rule-based supervised detection, typical of many deployed systems in practice. We demonstrate \method's efficacy through a series of case studies with fraud analysts from the financial industry.

==> 04eval_old.tex <==
\subsection{Simulation}
To assess the accuracy of our feature importance estimation in the anomaly detection scenario, we first outline our simulation method which involves creating anomalies from normal data and determining the impact of anomaly features by its deviation from the normal data. The goal of synthesizing anomalies is two-fold. One is to address the shortage of available public anomaly explanation datasets, which typically require a lot of human effort to annotate  anomalies and identify their causes. The other is to account for subjectivity, as people may have different perspectives on what features are important, making it difficult to establish a definitive feature importance (or ground truth). This is particularly the case for tabular %and streaming 
data, where anomaly features are harder to identify than anomalies of image pixels or video frames.

%\leman{unify the use of outlier or anomaly - dont use both. below you use anomaly. in the paper i use anomaly only.}
There are various techniques for generating anomalies, with many recent works utilizing deep generative architectures to produce realistic anomalies in tabular data, images, and other types of data with complex structural models \cite{altman2019,schluter2022self}.
\textcolor{blue}{We select a variational autoencoder (VAE) as the primary generative model to reflect the complex data distribution because we are analyzing anomalous explanations in data with both real and categorical features.}
%Since we are evaluating anomaly explanations on data with both real and categorical features, we choose a variational autoencoder (VAE) as the backbone generative model.
The VAE contains an encoder-decoder couple, parameterized by $\phi$ and $\theta$ respectively. It encodes  a training data point $\textbf{x}$ into a lower-dimensional $\textbf{z}$. At training stage, the encoder minimizes the distance of a surrogate posterior $q_\phi (\textbf{x} | \textbf{z})$ to the true  $p_\theta (\textbf{z})$, while the decoder maximizes $p_\theta (\textbf{x} | \textbf{z}) $, the probability of $\textbf{x}$ %'s appearance 
given sampling from $\textbf{z}$. With a trained VAE model, the likelihood of a point being an anomaly can be determined by its reconstruction probability $p_\theta (\textbf{x} | \textbf{z})$, with a higher probability indicating that it is more likely to belong to the normal %group of 
points. VAE not only generates realistic normal data points, but also assigns a probability score to the synthetic outliers, indicating how unusual they are.

%\leman{you want walk-through/reference lines in the algo (add line numbers!); after each sentence by e.g. (lines 1-4) etc.} 
Algo.\ref{alg:cap} describes the  details of our anomaly simulation algorithm. First, given an anomaly detection dataset, we feed all the normal points into a VAE model (Line \ref{lst:line:1}). In our experiments, we use the Gaussian prior $\mathcal{N}(0,1)$ for VAE. However, VAEs can be customized to fit the distribution of the training data by using different priors such as Gaussian Mixture Model \cite{dilokhanakuldeep2016}, VampPrior \cite{storkey2018vaevamp}, and etc. This can help achieve a good estimation of the underlying distribution and minimize training loss. A trained VAE can be used to generate $m$ normal points $\{\textbf{x}_{nor,i}\}_{i=1}^{m}$ with hidden variable $\textbf{z}_i$ (Line \ref{lst:line:2}), which can be useful e.g. for large $m$ when the original dataset is small. The threshold $\tau$ for identifying normal points is defined using the generated points as the minimum likelihood of a point being normal (Line \ref{lst:line:3}).
\begin{align}
\tau = \epsilon *  \min_{i=1,...,m}[ \log p_{\theta}(\textbf{x}_{nor,i} | \textbf{z}_i) ].
\end{align}

The threshold can be adjusted by controlling the value of the parameter $\epsilon$, which determines the tightness of the threshold.  

To generate an anomaly point, we sample another normal instance $\textbf{x}$ with hidden representation $\textbf{z}$, and decoder's score $\log p_\theta (\textbf{x} | \textbf{z})$ (Line \ref{lst:line:6} - \ref{lst:line:7}). We select a subset of features, and with each feature selected,   we ``inflate''  point $\textbf{x}$ among one specific dimension (Line \ref{lst:line:9}). There are several ways to inflate a point. When the feature is real-valued, a point can be placed in a low-density region that is far from the rest of the normal points (global anomaly) or in the surrounding region of the normal points but with low probability of appearance (local anomaly). When the feature is categorical, a point's feature can be changed by placing it into a feature class value with a lower probability according to the empirical categorical distribution. Let us denote the inflated point $\textbf{x}^\prime$. For $\textbf{x}^\prime$, a feature's explanation is computed (Line \ref{lst:line:10}) by the probability
\begin{align}
\log p_\theta(\textbf{x}^\prime | \textbf{z} ) - \log p_\theta ( \textbf{x} | \textbf{z} ) \;.
\end{align}
This probability describes how changing a feature, under the same hidden representation $\textbf{z}$, can cause a point to move from the normal cluster to becoming an anomaly. \textcolor{blue} {We use this change of probability as the feature importance weight.}
Then, we replace $\textbf{x}$ with all the previously inflated values, and denote it as $\textbf{x}_\text{candidate}$ (Line \ref{lst:line:12}). The candidate is kept if its posterior probability $ \log p_{\theta} (\textbf{x}_{\text{candidate}} | \textbf{z})$ falls into the lower probability region and is smaller than the threshold $\tau$. \textcolor{blue}{If $\textbf{x}_\text{candidate}$ is kept, we also build its associated feature importance weights, which is the list of difference in probabilities (for successfully inflated features) and zeros (for not-inflated features) (Line \ref{lst:line:13} - \ref{lst:line:15}). } 

\textcolor{blue}{The VAE-based approach offers several benefits compared to other methods. Firstly, VAE generates more realistic anomalies than simply creating synthetic points from predefined distributions. Secondly, VAE's posterior probability can determine if a point is in a low probability region, whereas randomly altering features may not necessarily change a point from normal to anomalous. Thirdly, the variations in posterior probability is a useful measurement of feature importance, as it indicates how much changing a feature results in an anomalous point.}

\leman{you have not 1) discuss why VAE and not other simple/vanilla/layman approach(es)? also 2) you have not mentioned what constitutes feature importance \textit{weights} exactly, based on this VAE model.}

\leman{i changed the title a bit. you are not generating explanations. explanations are in the form of feature importance (weights). so you are generating anomalies with ground-truth feature importances.}
\begin{algorithm}
\caption{Anomaly \& Feature Importance  Synthesis %and Explanation Generation
}\label{alg:cap}
\begin{algorithmic}[1]
\Require $n$ Real normal data points, $m$: number of generated normal points, $r$: number of anomalies, $\epsilon$: threshold, $d$: inflating features %\leman{avoid/get rid of orphan-words}
\Ensure $\{\textbf{x}_{nor,i}\}_{i=1}^{m}$ synthetic normal data, $r$ synthetic anomalies with feature importances.
\State Train a VAE model $VAE(\phi, \theta)$ on the $n$ normal data points. \label{lst:line:1}
\State Sample $\{\textbf{x}_{nor,i}\}_{i=1}^{m} \sim VAE(\phi, \theta)$ with $\{\textbf{z}\}_{i=1}^{m}$. \label{lst:line:2}
\State Set threshold $\tau \gets \epsilon \times  \min [ \log p_{\theta}(\textbf{x}_{nor,i} | \textbf{z}_i) ]_{i=1}^{m} $.
\label{lst:line:3}
\State Intialize empty AnomalyDataList, ExplainList and ScoreList.
\label{lst:line:4}
\While{len(AnomalyDataList) $< r$} \label{lst:line:5}
    \State Sample a $\textbf{x} \sim VAE(\phi,\theta) $with $\textbf{z}$. \label{lst:line:6}
    \State Initialize a vector $\textbf{e}$ of zeros, with equal size of $\textbf{x}$. \label{lst:line:7}
    \For{(feature $j \in d$)} \label{lst:line:8}
        \State Inflate feature $j$ of $\textbf{x}$ and get $\textbf{x}^\prime$. \label{lst:line:9}
         \State Let $\textbf{e}_j \gets \max [0, \log p_{\theta} (\textbf{x}^\prime | z) - \log p_{\theta} (\textbf{x} | z)]$.
         \label{lst:line:10}
    \EndFor \label{lst:line:11}
    \State Replace $\textbf{x}$ with all previously inflated features, denote as $\textbf{x}_{\text{candidate}}$. Compute $s \gets \log p_{\theta} (\textbf{x}_{\text{candidate}} | z) - \log p_{\theta} (\textbf{x}| z) $.
    \label{lst:line:12}
    \If{ $s < \tau$}   \label{lst:line:13}
     \State AnomalyDataList.append($\textbf{x}_{\text{candidate}}$). \label{lst:line:14}
        \State ExplainList.append($e$).   \label{lst:line:15}
\EndIf \label{lst:line:16}
\EndWhile \label{lst:line:17}
\State \Return $\{\textbf{x}_{nor,i}\}_{i=1}^{m}$, AnomalyDataList, ExplainList. \label{lst:line:18}
\end{algorithmic}
\end{algorithm}

\subsection{Experiment Setup} 

{\bf Data:~} 
We evaluate our anomaly explanation-by-feature importances approach on three real-valued and three mixed-type datasets, which are commonly used in anomaly detection literature for tabular data.
Table \ref{tab: datasetoverview} lists the dataset names and descriptions. \textcolor{blue}{All data are publicly available at UCI machine learning repository\cite{Dua2017UCI}. \footnote{downloadable at: \url{http://odds.cs.stonybrook.edu}}}

%\leman{any pointers? links? or citations? where one can find them--for reproducing.}

For each dataset, we pre-process the data by removing any points with missing features and any features that only have one value. We then use all the cleaned normal points to fit a VAE and generate 5000 normal points and 500 anomaly data points. \textcolor{blue}{To generate each anomaly, we inflate 1/3 of the dataset's features. The 1/3 of the features are randomly chosen for each anomaly. If one feature is real-valued feature, it can be inflated into either global or local anomaly feature. If it is a categorical feature, it is inflated to the class value with the lowest-probability.} 
%For the 500 anomalies, 1/3 of the total features are inflated, with some randomly turned into global and local outlying features and the lowest-probability for categorical features. \leman{the previous sentence is off, confusing, vague or poorly worded. revise/clarify.} 
%Anomaly scores and explanations \leman{(i.e. feature importance weights) -- but you did not exactly specify this. see my previous comment}%
\textcolor{blue} {The associated feature importance weights are obtained using our anomaly synthesis method and used as the ground truth for evaluating the explanations.}

%\leman{make the below table wraptable around the text above to save some space. Type can shrink to Mixed vs Real-val.}

\begin{wraptable}{r}{5.5cm}
\centering
\caption{Dataset statistics. }
\vspace{-0.15in}
	\centering
	\hspace{-0.1in}
	{\scalebox{1.0}{
    \begin{tabular}{lrrrr}
    \toprule
    \textbf{Name} &  \textbf{Type} &
    $|\mF_c|$
    %\textbf{Cat. dim.} 
    &   %\textbf{Cont. dim.}
    $|\mF_r|$ \\
    \midrule
    Seismic & Mixed &  4 & 11 \\
    KDDCUP & Mixed &  3 & 31 \\
    Hypothyroid & Mixed &  12 & 6 \\
    Cardio & Real-val & 0 & 21 \\
    Satellite & Real-val & 0 & 36 \\
    BreastW & Real-val & 0 & 9 \\
    \bottomrule
    \end{tabular}
}}
    \label{tab: datasetoverview}
\end{wraptable} 

\smallskip \noindent 
{\bf Baselines:~} 
We evaluate our method along with two state-of-the-art methods: SHapley Additive exPlanations (SHAP) \cite{lundberg2017unified} and Depth-based Isolation Forest Feature Importance (DIFFI)\cite{diffi2022carletti}. SHAP is a method for interpreting the output of any machine learning model that is based on Shapley values and is model-free. In constrast, DIFFI is a feature importance method that is specifically based on using Isolation Forest as the anomaly detection method. SHAP's feature importance can be obtained by using the prediction results of Isolation Forest and \ex. DIFFI's results are also based on training Isolation Forest as the backbone algorithm. 

We also evaluate feature importance using \ex with projection, using dimensionality $K$ of $15$, $20$, and $30$, as well as using \ex without projection. For \ex, we fix the $| \mathcal{M}_u | = 200$, and each chain's depth equals to $20$. The CMS hashtable size $m = 10$. \textcolor{blue}{We use these values as they are sufficiently large numbers to obtain good detection performance in \cite{manzoor2018xstream}.}

%\leman{size of CMS tables? maybe finish by saying these are sufficiently large numbers to obtain good detection performance and cite Emaad's paper.}

\smallskip \noindent 
{\bf Metrics:~} 
The metrics for evaluation are ranking based, quantifying how well we rank all features by importance; namely 
Normalized Discounted Cumulative Gain (NDCG) \cite{ndcg2000} and Kendall's rank correlation coefficient (Kendall's Tau) \cite{kendall1938rank}. NDCG compares the effectiveness of a ranking to an ideal ranking, and summing the weighted scores of the items in the predicted ranking. It ranges between $0$ and $1$. Kendall's Tau is between $-1$ and $1$. It evaluates the similarity between two rankings, by counting the number of concordant pairs and discordant pairs among every two variables of the ranking.



\subsection{Results}
Table \ref{tab:ndcg} and Table \ref{tab:kendalltau} respectively show the NDCG and Kendall's Tau scores of the compared methods,  in comparison to the synthesized ground-truth explanations. We observe that XPACS \ex (without projection) achieves comparable performance to state-of-the-art explanation models in many datasets, with high NDCG and Kendall Tau scores. \leman{comparable meaning barely matches? does it not outperform?}
However, there is no single combination of anomaly detection and explanation methods that consistently performs better than others, across all datasets. \leman{ok so we can use any one of them? why did we create a new approach if others are equally good?} 
\leman{i dont see the value your proposed explanation method has over existing baselines... is it speed? performance? what is it? why propose something new that is only barely comparable to existing stuff?!}

\leman{projection is a different conversation.}The use of projection diminishes XPACS' capability to identify and explain anomalies. When projection is used on the underlying data, there is a noticeable decrease in both scores. Despite this, the use of projection allows XPACS to explain evolving and streaming data without requiring a complete retraining of the algorithm, making it more suitable for deployment in real-time applications.


We also plot the variations among different method's explanations in Fig. (planning to insert a confusion matrix plots). We demonstrate that even when using a single dataset, the combination of different anomaly detection methods and feature importance explanations can result in significant variations in the rankings of feature importance. As a result, there is no universally ``best'' feature explanation that can be considered the definitive truth or rule for end-users. \leman{so why did you propose a new explanation method?} This outcome highlights the significance of developing a toolkit for managing anomalies: rather than blindly accepting the feature importances produced by any specific algorithm, analysts should be able to actively participate in the process of rule mining and become involved in the anomaly mining and management cycle.   

\begin{table*}[h]
\caption{NDCG Score}
\begin{tabular}{c c c c c c c}
\hline
{Method} & {Seismic} & {KDDCUP} & {Hypothyroid} & {Cardio} & {Satellite} & {BreastW} \\
\hline
IF+SHAP & 
0.857$\pm$0.002 &
0.740$\pm$0.010 & 
0.806$\pm$0.015 & 
0.820$\pm$0.115 & 
0.911$\pm$0.001 &
0.957$\pm$0.008 \\
IF+DIFFI &
0.877$\pm$0.013 & 0.725$\pm$0.008 & 0.824$\pm$0.023 & 0.824$\pm$0.047 & 0.867$\pm$0.005 & 
0.912$\pm$0.006 \\
XPACS(No Proj.) & 
0.873$\pm$0.018 & 0.670$\pm$0.010 & 0.835$\pm$0.020 & 0.836$\pm$0.008 &
0.912$\pm$0.006 &
0.834$\pm$0.005 \\
XPACS+SHAP &
 &
 &
 &
&
&
\\
\hline
XPACS(Proj.=15) &
 0.666$\pm$0.006&
 0.457$\pm$0.006 &
 0.532$\pm$0.005&
 0.706$\pm$0.005& 
0.672$\pm$0.006&
0.850$\pm$0.004 \\
XPACS(Proj.=20) &
0.702$\pm$0.002&
0.472$\pm$0.005&
0.560$\pm$0.008&
0.713$\pm$0.009&
0.655$\pm$0.004&
0.870$\pm$0.005 \\ 
XPACS(Proj.=30) &
0.718$\pm$0.003 &
0.488$\pm$0.006&
0.559$\pm$0.007 &
0.752$\pm$0.005&
0.690$\pm$0.007&
0.881$\pm$0.004\\
\end{tabular}
\label{tab:ndcg}
\end{table*}

\begin{table*}[h]
\caption{Kendall Tau Score}
\begin{tabular}{c c c c c c c}
\hline
{Method} & {Seismic} & {KDDCUP} & {Hypothyroid} & {Cardio} & {Satellite} & {BreastW} \\
\hline
IF+SHAP & 
0.376$\pm$0.002 &
0.311$\pm$0.002 & 
0.340$\pm$0.004 & 
0.333$\pm$0.004 & 
0.478$\pm$0.002 &
0.563$\pm$0.002 \\
IF+DIFFI &
0.357$\pm$0.002 & 
0.126$\pm$0.023 & 
0.361$\pm$0.035 & 
0.287$\pm$0.005 & 
0.348$\pm$0.009 & 
0.383$\pm$0.004 \\
XPACS(No Proj.) & 
0.409$\pm$0.011 & 
0.185$\pm$0.012 & 
0.559$\pm$0.011 & 
0.340$\pm$0.001 &
0.491$\pm$0.005 &
0.428$\pm$0.004 \\
XPACS+SHAP &
 &
 &
 &
&
&
\\
\hline
XPACS(Proj.=15) &
 0.112$\pm$0.003&
 0.085$\pm$0.002 &
0.041$\pm$0.002 &
 0.133$\pm$0.003& 
 0.060$\pm$0.002&
0.268$\pm$0.001 \\
XPACS(Proj.=20) &
0.131$\pm$0.005&
0.084$\pm$0.002&
0.063$\pm$0.004&
0.131$\pm$0.004 &
0.056$\pm$0.002&
0.285$\pm$0.008 \\ 
XPACS(Proj.=30) &
0.125$\pm$0.001 &
0.085$\pm$0.002&
0.064$\pm$0.002&
0.140$\pm$0.001&
0.072$\pm$0.002&
0.270$\pm$0.002\\
\end{tabular}
\label{tab:kendalltau}
\end{table*}

==> algostep1.tex <==



\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\renewcommand{\algorithmiccomment}[1]{\hfill$\blacktriangleright$ #1}
%\newcommand{\cdash}{\multicolumn{1}{c}{--} }
\newcommand{\algrule}[1][.5pt]{\par\vskip.5\baselineskip\hrule height #1\par\vskip.5\baselineskip}
\makeatother

%\algnewcommand{\IIf}[1]{\STATE\algorithmicif\ #1\ \algorithmicthen}
%\algnewcommand{\EndIIf}{\unskip\ \algorithmicend\ \algorithmicif}

\begin{algorithm}[!t]

	\caption{\method \textbf{Step 1.} Distributed Data Projection }
	\label{algo:step1}
	\begin{algorithmic}[1]
			\small{
		\REQUIRE  inputDF (input data), $K$ (proj. dim.), featureNames
		\ENSURE projDF ($K$-dimensional transformed \df)
		\algrule
		\STATE projector = HashProjn($K$,  seeds=arange$(0, K, 1)$, density=1/3)	
		\STATE  projDF = inputDF.{\textcolor{blue}\map}(lambda $x$: projector.{\tt fit\_transform}($x$) 
		\algrule
		
		 {\bf procedure} {\tt fit\_transform}($pt$)
				\STATE \hspace{0.1in} {{\bf for each} $F$ in featureNames:} 
				\STATE \hspace{0.2in} {{\bf if} $F$ is categoric} {\bf then }
					 $F:= F \oplus pt[F]$  
			
				\STATE \hspace{0.1in} $R =$ array([[{\tt hash\_string}$(k, str)$ 
					 for $k$ in seeds]
				\STATE \hspace{1.78in} for $str$ in featureNames])
			
			\STATE \hspace{0.1in} {\bf return}	 proj\_$pt$ =  $R \cdot pt$ 
		 \COMMENT{dot product}	
		}			
	\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{0.05in}
% \pagebreak










==> algostep2.tex <==


\begin{algorithm}[!t]
	\caption{\method \textbf{Step 2.} Distributed Half-space Chains}
	\label{algo:step2}
	\begin{algorithmic}[1]
			\small{
		\REQUIRE projDF, $L$ (chain-length), sampleRate, numRows, numCols,  numChains, numThreads
		\ENSURE  CMSketches (counts at all levels $l=1\ldots L$ per chain) 
		\algrule
		{\bf procedure} {\tt fit\_chain}(seed)
		\STATE \hspace{0.1in}C = Chain($\bdel$, $L$)
		\STATE \hspace{0.1in}binIDsDF = projDF.rdd.sample(sampleRate, seed)
		\STATE \hspace{0.92in}.{\textcolor{blue}\map}(lambda $x$: C.{\tt fit}($x$))
		
		\STATE \hspace{0.1in}cms = CMS(numRows, numCols)
		\STATE \hspace{0.1in}{\bf for} $l$ in range($L$):
		\STATE \hspace{0.2in}C.CMSketches[$l$] = binIDsDF
		\STATE \hspace{0.4in}.{\textcolor{blue}{\tt flatMap}}(lambda $x$: cms.{\tt allCols}($x[l]$))
		\STATE \hspace{0.4in}.{\tt \textcolor{red}{reduceByKey}}(lambda a,b : a+b)
		%\STATE 
		%\hspace{0.9in}
		.{\tt collectAsMap}()
	%	\STATE \hspace{0.1in}Chains.append(C)
		\algrule
		\STATE tpool = ThreadPool(numThreads)
		\STATE  indxlist = list(range(numChains))
		\STATE  tpool.{\textcolor{blue}\map}(lambda cind: {\tt fit\_chain}(cind), indxlist)
	
		% \COMMENT{\S\ref{}}	
	}			
	\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{0.05in}
% \pagebreak


==> algostep3.tex <==





\begin{algorithm}[!t]
	\caption{\method \textbf{Step 3.} Distributed Outlier Scoring}
	\label{algo:step3}
	\begin{algorithmic}[1]
			\small{
		\REQUIRE projDF, CMSketches (for all chains)
		\ENSURE  outlier\_scores
		\algrule
		{\bf procedure} {\tt score\_chain}(cindex, CMS)
			\STATE \hspace{0.01in} C = Chains[cindex]
			\STATE \hspace{0.01in} scoreC=projDF.{\textcolor{blue}\map}(lambda $x$:C.{\tt score}($x$, CMS.value[cindex]))
			%\STATE \hspace{1.12in} 
			
		\algrule
		\STATE CMS = sc.broadcast(CMSketches)
		\STATE tpool = ThreadPool(numThreads)
		\STATE  idx = list(range(numChains))
		\STATE  outlier\_scores = {\tt sum}(tpool.{\textcolor{blue}\map}(lambda c: {\tt score\_chain}(c), idx))
		% \COMMENT{\S\ref{}}	
	}			
	\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{0.05in}
% \pagebreak


==> old-06results.tex <==


\subsection{Results}
\label{ssec:results}

\subsubsection{\bf \dbs does not scale w.r.t. dimensionality $d$.~} %\la{[Plot 5]}
We start with analyzing results on our small-$n$/large-$d$ \gis. First, we show that \dbs scales very poorly with increasing dimensionality using this moderately large dimensional dataset. 

\begin{table}[!t]
	\caption{\dbs scales poorly with $d$. On \gis, running time grows fast from $d$$=$1 to 10, and then %features, after which the implementation 
		times out.}  
	\label{tab:dbsdim}
	\vspace{-0.15in}
	\centering
	\scalebox{0.85}{
		\begin{tabular} {l|rr} 
			\toprule
			\textbf{$d$ dim.} &  \textbf{Runtime (sec)} & \textbf{Peak memory (MB)}  \\ 
			\midrule
%			1                    & 13.5                        & 1,630                 \\
			2                    & 11.3                        & 1,650                 \\
			4                    & 13.0                          & 1,630                 \\
%			5                    & 17.7                        & 1,660                 \\
			6                    & 31.1                        & 133,000               \\
%			7                    & 111.6                       & 130,000               \\
			8                    & 429.8                       & 254,000               \\
			10                   & 3,420.0                        & 350,000               \\
			11                   & {TIMEOUT} & N/A \\
			\bottomrule
		\end{tabular}
	}
\vspace{0.05in}
\end{table}

As shown in Table \ref{tab:dbsdim}, when using \congen, the running time grows dramatically fast as we run \dbs on \gis using an increasing number of randomly sampled 1--10 features. It reaches around 60-min mark at only $d$$=$10, and with 11 features, the process times-out (after 8 hrs). 
Peak memory usage responds similarly growing from 1.6GB to a total of 350GB across the executors.



Poor scalability makes \dbs infeasible for datasets with more than a handful of features, therefore we only report results on \gis for \method and \dif. 
%, and compare to \dbs on \open, which was also used in their original paper (along with other 2-d or 3-d datasets).


\vspace{-0.05in}
\subsubsection{\bf Accuracy vs. Resources Landscape.~~} %\la{[Plots 1 \& 2]}
Next we analyze the trade-off between detection quality and resources required. 
Fig. \ref{fig:gis} shows AUROC (y-axis) versus total running time (x-axis, left) and peak driver memory (x-axis, right) under 
\congen. We find that \dif performance varies between 0.72-0.80 across HP configurations whereas \method reaches 0.80-0.87. On the other hand, \method uses more resources; as compared to \dif's typical runtime 1-2 minutes, \method can achieve its peak performance in around 14 minutes, using 2-3$\times$ more memory.
Similar conclusions are drawn under
\conmod, which is in Appx. \ref{sssec:gis}, Fig. \ref{fig:gis2}.
%In Appx. Table \ref{tab:h2h}, we also present a more ``head-to-head'' comparison under comparable settings of the HPs for both methods.

\begin{figure}[!ht]
		\vspace{-0.1in}
	\centering
\hspace{-0.1in}	\includegraphics[width=0.4995\linewidth]{FIG/gis-scatter-time-c3}
\hspace{0.00in}	\includegraphics[width=0.4995\linewidth]{FIG/gis-scatter-mem-c3}
		\vspace{-0.25in}
	\caption{Comparing \method (red) and \dif (blue) on \gis: (left) Running time (sec) vs. accuracy in AUROC, and (right) Peak driver memory (MB) vs. AUROC. Symbols depict different hyperparameter configurations. \dbs does not run on \gis due to dimensionality. \label{fig:gis}}
		\vspace{-0.15in}
\end{figure}

Table \ref{tab:h2h} presents a more ``head-to-head'' comparison under comparable settings of the HPs for both methods.
Increasing (doubling) the number of ensemble components improves \method's accuracy, with no effect on \dif; whereas it is vice versa when increasing the sampling rate. However, even with all data (sampling rate $=$ 1), \dif does not exceed an AUROC of 0.8. 
%For \gis, larger depth does not help with accuracy while increasing model size for \method (hence running time and memory as well). \dif model size does not change much with depth 20 vs. 10, as it is an upper-bound and tree construction is stopped when another criterion (min. pts. in leaf) is met.  

Importantly, notice that when the number of samples per tree goes up from 4,000 (rate$=$0.1) to 40,000 (rate$=$1), \dif's running time notably increases. This is due to its model-parallel yet {\bf not} data-parallel nature; where all samples per tree are shuffled (i.e. copied) over the network to a worker that is designated to construct the tree. With 100 trees, the total network communication becomes notable.
In fact, \dif quickly becomes infeasible to run on massive datasets even with a tiny subsampling rate, exactly due to this data shuffling problem, as we show in the next section.

\begin{table}[]
		\caption{``Head to head '' comparison of \method and \dif on \gis under equivalent hyperparameter configurations.}  
	\label{tab:h2h}
	\vspace{-0.15in}
	\centering
	\scalebox{0.825}{
	\begin{tabular}{lrrr|rr|rr|rr}
		\toprule
	&         &        &       &   \multicolumn{2}{c|}{AUROC} & \multicolumn{2}{c|}{Time(s)} & \multicolumn{2}{c}{Mem (MB)} \\ \hline
	conf.	& \#comp. & sampl. & depth &   Sx        &    DIF         &       Sx       &      DIF        &       Sx        &       DIF       \\
	\midrule
	1	&     \underline{50}		  &   0.01     &  10       &      0.80
	       &     0.77        &             610.5 &
	       58.0             &        230.2
	              &      99.6        \\
	2	&    \underline{100}     &       \underline{0.01}     &  10       &     0.85      &     0.76		     &      836.0          &   58.0           &        230.7        &      99.0        \\
	3	&   100     &       \underline{0.1}     &  \underline{10}        &     0.86		        &    0.79		         &    874.2          &      61.1        &     229.9          &     102.8         \\
	4	&     100     &       \underline{0.1}     &  \underline{20}        &      0.87		       &    0.78		         &    1455.6          &          60.1    &        334.5       &       99.0       \\
	5	&    100     &       \underline{1}     &  20       &     0.85		        &    0.80	         &     2312.8         &       111.0       &         360.8      & 	101.1 \\
	\bottomrule           
	\end{tabular}
}
\end{table}


\vspace{-0.05in}
\subsubsection{\bf \dif does not scale w.r.t. input size $n$.~} %\la{[Plot 4]}
As a reminder, a key design principle in distributed computing on big data is ``\textit{code goes to data}'' and {\bf not} vice versa. In other words, the goal is to compute as much as possible {\em locally} and not to move around data between compute nodes (other than data containing intermediate results).
The way \dif is implemented violates this principle and suffers on large-scale data. We demonsrate the problem using \open.


Using \congen, we input to \dif\footnote{We set model HPs as num\_trees=50, max\_depth=25, and sample\_rate=0.01.} a gradually increasing fraction of \open (for \textit{fitting}, while all 2.7+ billion points are scored), starting only with around 1/1000'th of the data, as shown in Table \ref{tab:difvsn}. 
As we double the input size at every round, total running time and memory usage increase accordingly.
However, when the number of points per tree reaches around half a million, we get a system memory error and the program crashes.
As we continue to increase data size, data processing cannot reach the memory error before the 8-hour SC-budget is exhausted and we get a system time-out.


\begin{table}[H]
	\vspace{-0.1in}
	\caption{\dif does not scale up w.r.t. input size $n$.} % on \open.} %resource usage by increasing input size of \open.}  
	\label{tab:difvsn}
	\vspace{-0.15in}
	\centering
	\scalebox{0.85}{
\begin{tabular}{rrrrrr}
\toprule
\multicolumn{1}{l}{Frac.}   & \multicolumn{1}{l}{\#pts/tree} & Time (s)                 & Mem (GB)                & AUPRC                    & AUROC                    \\
\midrule
\multicolumn{1}{l}{0.00128} & 35,471                          & \multicolumn{1}{r}{1396} & \multicolumn{1}{r}{454} & \multicolumn{1}{r}{0.19} & \multicolumn{1}{r}{0.987} \\
\multicolumn{1}{l}{0.00256} & 70,943                          & \multicolumn{1}{r}{1402} & \multicolumn{1}{r}{455} & \multicolumn{1}{r}{0.27} & \multicolumn{1}{r}{0.989} \\
0.00512                     & 141,887                         & \multicolumn{1}{r}{1531} & \multicolumn{1}{r}{461} & \multicolumn{1}{r}{0.38} & \multicolumn{1}{r}{0.991} \\
0.01024                     & 283,774                         & \multicolumn{1}{r}{1834} & \multicolumn{1}{r}{463} & \multicolumn{1}{r}{0.42} & \multicolumn{1}{r}{0.993} \\
0.02048                     & 567,548                         & MEM ERR                  & -                       & -                        & -                         \\
0.04096                     & 1,135,097                        & MEM ERR                  & -                       & -                        & -                         \\
0.08192                     & 2,270,194                        & TIMEOUT                  & -                       & -                        & -                         \\
0.16384                     & 4,540,389                        & TIMEOUT                  & -                       & -                        & -              \\          
\bottomrule
\end{tabular}
}
\vspace{-0.15in}
\end{table}
%\la{moderate vs generous??}

As we have done, it is possible to fit \dif on a small subsample of a massive dataset -- to avoid this error during fitting -- and still be able to \textit{score} \textit{all} data points. However, as Table \ref{tab:difvsn} shows this incurs a sacrifice in detection performance (note esp. the AUPRC). %, which increases by using more data for model training.





\subsubsection{\bf Large-$n$/Small-$d$.~}
%\la{Plots 1 \& 2 for all 3 methods on \open. }
Next we analyze the results on \open, containing billions of points but only 2 dimensions.
Fig. \ref{fig:open} shows the landscape of detection performance (F1) vs. resources used for all three methods, under varying HP configurations. (See Appx. \ref{sssec:osm}, Tables \ref{table:spif-osm-3}--\ref{table:sparx-osm-3} for detailed numbers.)
Note that \dbs outputs a binary label, thus we can only report F1 for comparison.\footnote{Detailed numbers in Appx. include AUROC and AUPRC for \dif and \method.}

\dif can be fit using at most $10^{-4}$-th of the data, as discussed earlier, which results in very poor performance (F1$<$0.2).
\dbs is the fastest on this low-$d$ setting and achieves the most competitive performance, however, it is quite sensitive to the HP choices and its performance oscillates widely.
\method performance is more stable, with a longer processing time, while  using less memory. 



\begin{figure}[!t]
%	\vspace{-0.1in}
	\centering
	\hspace{-0.1in}	\includegraphics[width=0.4995\linewidth]{FIG/osm-scatter-time-c3}
	\hspace{0.00in}	\includegraphics[width=0.4995\linewidth]{FIG/osm-scatter-mem-c3}
	\vspace{-0.3in}
	\caption{Comparing all methods on \open under \congen: (left) Running time (sec) vs. accuracy in F1, and (right) Total memory (GB) vs. F1. Symbols depict different HP config.s.  \label{fig:open}}
%	\vspace{-0.1in}
\end{figure}



%can only compare w.r.t. F1
%Appx. Table ? includes AUROC and AUPRC for \dif and \method.

\vspace{-0.05in}
\subsubsection{\bf Large-$n$/Large-$d$.~}
Finally, we present a similar analysis on our very large-$d$ (yet sparse) \surl.
Problematically, the
\dif implementation cannot handle sparse RDD input (and it is infeasible to store \surl as a dense RDD).
Therefore, we transform it using our random projections to $d$=100. (Our \method also uses $K$=100 projections.) 
\dbs scales very poorly with dimensionality, for which we also transform \surl to $d$=7 (largest $d$ that \dbs could handle), as well as $d$=2 (for comparison).

\begin{figure}[!ht]
	\vspace{-0.15in}
	\centering
	\hspace{-0.1in}	\includegraphics[width=0.51\linewidth]{FIG/spam-scatter-time-c3}
	\hspace{-0.1in}	\includegraphics[width=0.51\linewidth]{FIG/spam-scatter-mem-c3}
	\vspace{-0.1in}
	\caption{Comparing methods on \surl under \congen: (left) Running time (sec) vs. accuracy in F1, and (right) Total memory (GB) vs. F1. Symbols depict different HP config.s.  \label{fig:spam}}
	\vspace{-0.1in}
\end{figure}


As shown in Fig. \ref{fig:spam}, \dbs with $d$=2 is quite resource-frugal, however it has a widely varying performance depending on the choice of hyperparameters. It achieves more stable performance with $d$=7, yet is inferior to \dif in both time and accuracy.
On the other hand, 
\method performance is robust to different hyperparameter settings, and is on par with the competing baselines.  

%\la{on \surl: how does \dif do? how does \dbs do {\em after projecting to d=10}?}
%\la{Plots 1 \& 2 for all 3 methods on \surl. }


\vspace{-0.05in}
\subsubsection{\bf Speed-up by increasing parallelism.~} %\la{[Plot 3]}

Next we show how \method leverages data-parallelism, Using \gis, we increase the number of DataFrame partitions on Spark. 
Fig. \ref{fig:speedup1} shows that  the running time decreases as partitions increase from 8 to 128, and then slightly increases for 256. This is expected behavior of distributed platforms---that speed-up is not monotonic: when the data is partitioned too much to the extent that each worker is under-utilized, the cost of network communication between workers overtakes and reduces the gains from parallelism. As compared to the running time of single-machine \ex, \method provides 4-20$\times$ speed-up.
%\la{Plot 3 on \gis for \dif and \method. \dif does not pay off. Thus, repeat on \open -- for all 3 methods }
\begin{figure}[!th]
		\vspace{-0.1in}
	\centering
	\includegraphics[width=0.7\linewidth]{FIG/gis-doubley-sparx}
		\vspace{-0.15in}
	\caption{(in blue) Running time of \method on \gis as number of data partitions increases. (in red) Speed-up w.r.t. single-machine implementation. \label{fig:speedup1}}
			\vspace{-0.15in}
\end{figure}

\vspace{-0.05in}
\subsubsection{\bf \method scalability with input size $n$.~} %\la{[Plot 4 for \method]}
%\la{wrap up. Plot 5 (scalability by $d$) for \method not needed,  projection is linear?}
Finally, we study the scalability of our distributed \method w.r.t. input size. 
Recall that dimensionality $d$ is associated with Step 1. (projection) of the algorithm, where in Sec. \ref{ssec:st} we have shown that \method is linear in $d$. We have also shown that across all 3 steps, it is linear in the number of data points $n$. Since Spark-like platforms are distributed/data-parallel in $n$, we study the running time of \method for increasing sizes of $n$ using \open.\footnote{We set model HPs as num\_chains=10, depth=5, and sample\_rate=1.} As shown in Fig. \ref{fig:scalebyn}, \method scales linearly w.r.t. $n$, emprically confirming our complexity analysis in Sec. \ref{ssec:st}.
%\reminder{which config, what hyperparams}
\begin{figure}[!t]
		%\vspace{-0.15in}
	\centering
	\includegraphics[width=0.6\linewidth]{FIG/scale-by-n}
	\vspace{-0.15in}
	\caption{\method scales linearly in number of points $n$. \label{fig:scalebyn}}
		%	\vspace{-0.15in}
\end{figure}



{\bf Summary and remarks.} % discuss 
%\la{ \dbs fails for Plot 5. \dif fails on Plot 4.}
To sum up, through extensive experiments we showed that \method applies to all large-$n$ and/or large-$d$ datasets,  provides competitive detection accuracy-running time trade-off, takes advantage of data parallelism effectively, and scales up with increasing input size. In contrast, among the handful of public-domain distributed OD algorithms, (1) \dbs \textbf{has poor scalability w.r.t. dimensionality $d$}, being applicable to only small-$d$ ($d$$<$$10$) datasets in practice. On the other hand, (2) \dif \textbf{cannot handle large-$n$ datasets} due to its non-data-parallel implementation, also rendering it a non-practical choice. 







